CCTEST: Testing and Repairing Code Completion Systems

Code completion, a highly valuable topic in the software development domain, has been increasingly promoted for use by recent advances in large language models (LLMs). To date, visible LLM-based code completion frameworks such as GitHub Copilot and GPT are trained using deep learning over vast quantities of unstructured text and open source code. As the paramount component and the cornerstone in daily programming tasks, code completion has largely boosted professionals' efficiency in building real-world software systems. In contrast to this flourishing market, we find that code completion systems often output suspicious results, and to date, an automated testing and enhancement framework for code completion systems is not available. This research proposes CCTEST, a framework to test and repair code completion systems in blackbox settings. CCTEST features a set of novel mutation strategies, namely program structure-correlated (PSC) mutations, to generate mutated code completion inputs. Then, it detects inconsistent outputs, representing possibly erroneous cases, from all the completed code cases. Moreover, CCTEST repairs the code completion outputs by selecting the output that mostly reflects the "average" appearance of all output cases, as the final output of the code completion systems. We detected a total of 33,540 inputs (with a true positive rate of 86%) that can trigger erroneous cases from eight popular LLM-based code completion systems. With repairing, we show that the accuracy of code completion systems is notably increased by 40% and 67% with respect to BLEU score and Levenshtein edit similarity.

==> approach.tex <==
\section{Program Structure-Correlation (PSC) Testing}
\label{sec:approach-overview}
This research proposes a novel testing scheme, named program
structure-correlation (PSC) testing, to test decompilation correctness of
software decompilers. Our \textit{key observation} is that programs with
similar/identical control structures will retain such correlation in the
corresponding decompiled code (assume optimizations of compilers/decompilers
are \textit{disabled}). Hence, by observing certain decompiled code manifesting
inconsistent control structures, potential decompilation errors can be flagged.

\begin{figure*}
  \centering
  \includegraphics[width=0.70\linewidth]{fig/psc-testing.pdf}
  \caption{Workflow of program structure-correlation (PSC) testing by comparing
    $p^{*}_{0}$ and $p^{*}_{k}$.}
  \label{fig:psc}
\end{figure*}

\F~\ref{fig:psc} depicts the workflow of PSC testing. Starting from a seed
program $p_{0}$, we conduct a two-step approach to 1) performing
structure-correlation mutation to generate a set of mutated programs with
identical or similar control structures and collect the decompiled program
$p^{*}_{k}$ from each mutated program $p_{k}$, and 2) computing structure-level
distance by comparing each $p^{*}_{k}$ with $p^{*}_{0}$ derived from $p_{0}$. We
identify outlier $p^{*}_{i}$ such that its control structure has an abnormal
long distance compared to $p^{*}_{0}$; these outliers are deemed as wrong code
errors. We will manually confirm each divergent case and reduce false positives.
We now discuss two key challenges in conducting PSC testing.

\subsection{Generate Test Cases with Structure-Correlation Mutation}
\label{subsec:test-case-mutation}
To generate structure-correlation mutation, one can replace one code fragment
$s_{0}$ (e.g., a statement) in the seed program $p_{0}$ with similar fragments
$s_{i} \in S$. By providing a set of programs (e.g., compiler benchmarks), we
will leverage \textit{code embedding} methods (see the following paragraph) to
generate embedding vectors of fragments in each program; the extracted
embeddings will be kept for use. Then, given a program $p_{0}$ as the seed
input, we select one fragment $s_{0}$ from $p_{0}$ (suppose the embedding of
$s_{0}$ is $v_{0}$), and search for certain kept fragment $s_{i}$, such that its
corresponding embedding $v_{i} \approx v_{0}$ ($\approx$ can be decided by
computing distances of embedding vectors). These statements $s_{i}$ will be used
to replace $s_0$ and generate a set of mutated programs $p_{k}$. The mutated
programs are expected to exhibit similar or identical program structures
compared to $p_0$. In addition, one can also mutate variable types in each seed
program: type mutation shall retain syntactic structure in the mutated programs,
but impose direct challenges in the type recovery module of decompilers
(see \F~\ref{fig:psc-sample} for a decompiler flaw exposed via variable type
mutation).

We use code embedding techniques to convert each code fragment into a dense
numeric vector. Similar code fragments manifest similar or identical vectors in
terms of distance. Recent advancements in applying NLP techniques toward
software~\cite{alon2019code,feng2016scalable} has enabled the construction of
embeddings for programs, and the proposed embedding models have been
demonstrated to have promising results on related code comprehension tasks.

One key assumption of PSI testing is that programs with similar/identical
control structures shall result in decompiled programs of similar/identical
structures. Hence, we compare control structures of decompiled programs:
outliers of control structures presumably indicate a decompiler bug.


\subsection{Identify Erroneous Cases with Structure Distance Computation}
\label{subsec:identify-error}

For each decompiled output $p^{*}_{k}$, we compare it with the reference
$p^{*}_{0}$ and compute a program distance, indicating how different they
are~\cite{sun2016finding}. Program distance $\Delta$ of two program $P$ and $Q$
can be defined as follows:

$$\Delta(P,Q) = \alpha \cdot d(V_{Q}, V_{P}) + \beta \cdot d(E_{Q}, E_{P})
- \gamma \cdot |Q-P|$$

\noindent where $d(P,Q) = 1 - \dfrac{|P \cap
Q|}{|A \cup B|}$ is the Jaccard index, and $|Q-P|$ is the difference of program
size. $V_{P}$, $V_{Q}$ denote CFG node sets and $E_{P}$, $E_{Q}$ denote CFG edge
sets, respectively. $\alpha$ and $\beta$ are weights that can be decided by
users. The program distance is defined by subsuming both complex mutations in
terms of the program control graphs, and also simple changes by inserting or
deleting program statements. Therefore, a distance over threshold between
$p_{k}^{*}$ and $p_{0}^{*}$ indicates decompilation errors on $p_{k}^{*}$. Once
computing the distances, we rely on a thresholding $T$ to identify the error
($T$ will be decided with empirical evidences). We report the top-$k$ cases for
further investigation.

\begin{figure}[t]
  \centering \includegraphics[width=1.1\linewidth]{fig/emi-psi.pdf}
  \caption{Comparison of PSC testing scheme with a recent work~\cite{liu2020how}
  (referred to as EMI testing scheme in the rest of this paper).} ]
  \label{fig:comparison}
\end{figure}

\smallskip
\noindent \textbf{Comparison with EMI-based Decompiler Testing.}~~While the
existing EMI-based compiler/decompiler testing method~\cite{liu2020how} can
effectively identify errors by executing and comparing two programs of the same
input, we note that compilation/decompilation errors can be found, only when the
mal-functional code is covered during runtime. In other words, the EMI-based
technique has a high chance of missing certain defects (i.e., false negatives).

\F~\ref{fig:comparison} compares EMI testing with PSC testing techniques.
The PSC testing method outperforms EMI testing by performing a program-wide
comparison, and can potentially expose more wrong code errors. Nevertheless, EMI
testing has no false positive cases, while manual investigation is needed to
eliminate false positives in PSC testing. We will conduct an experimental
comparison in terms of these two testing methods.


==> evaluation-emi.tex <==
\subsection{Decompilation Defects}
\label{subsec:evaluation-deviant-outputs}
This section answers \textbf{RQ2}: \textit{what are the characteristics of
  typical decompilation defects?} \T~\ref{tab:results} classifies all the
deviant outputs into five categories. In the rest of this section, we elaborate
on typical errors within each category.

\subsubsection{Type Recovery}
\label{subsubsec:type-failure}
The lack of fool-proof type recovery is one key limit of existing decompilers.
While for C code, not all the type recovery failure breaks the semantics, in
this study we flag a considerable amount of recovered variable types breaking
semantics (in terms of both control and data flow). Consider an example below:

\vspace*{3pt}
\noindent\begin{minipage}{.50\linewidth}
\begin{lstlisting}
// source code
int i = 0;
for(i=6; i<-12; i-=6){
  ... // not reachable
}
\end{lstlisting}
\end{minipage}\hspace*{12pt}
\begin{minipage}{.50\linewidth}
\begin{lstlisting}
// decompiled code
unsigned int i = 0;
for(i=6; i<-12; i-=6){
 ... // reachable
}
\end{lstlisting}
\end{minipage}

\noindent where the Csmith-generated C code has a \keyword{for} loop, but will
execute for zero iterations. Contrarily, the type recovery incorrectly annotates
\texttt{i} with \keyword{unsigned int} in the decompiled C code, and the loop
body becomes reachable in the decompiled output. In other words, the type
recovery alters the \textit{control flow}, and further changes the semantics.

We also find a considerable amount of type recovery failure that leads to an
erroneous \textit{data flow}. Consider a case below found:

\vspace{3pt}
\noindent\begin{minipage}{.50\linewidth}
\begin{lstlisting}
// source code
int32_t a = 0xaaffff;
\end{lstlisting}
\end{minipage}\hspace*{12pt}
\begin{minipage}{.50\linewidth}
\begin{lstlisting}
// decompiled code
int16_t a = 0xaaffff;
\end{lstlisting}
\end{minipage}

In the decompiled output, the variable type \keyword{int32\_t} is incorrectly
recovered as \keyword{int16\_t}. As a result, \texttt{a} is initialized with a
different value, since a variable of \keyword{int16\_t} type can only take the
lowest 16 bits (0xffff).

As reported in \T~\ref{tab:root}, 315 type errors in C code decompiled by RetDec
root from two bugs (Bug$_{1}$ and Bug$_{4}$). Bug$_{1}$ happens by converting
signed \texttt{mov} statements (\texttt{movsx}) in x86 assembly into IR
statements without correctly considering extensions and truncations. Bug$_{4}$
missed certain function call parameters when analyzing the call site stack push
operations. Bug$_{8}$, Bug$_{11}$, and Bug$_{13}$ cause in total 35 type errors
in Radare2/Ghidra. Bug$_{8}$ cannot precisely infer the ``length'' of stack
variables, while Bug$_{11}$ performs constant propagation optimization and uses a
ghost variable defined in Ghidra of wrong type to replace original variables. As
aforementioned, Bug$_{13}$ lifts unsigned shift in IR into signed shift in C
code.

\subsubsection{Variable Recovery}
\label{subsubsec:variable-recovery}
We find 338 variable recovery issues from RetDec, where this decompiler seems
unable to recognize certain variables and future leads to deviant execution
outputs compared with the seed programs. Root cause analysis shows that
Bug$_{2}$, a bug on function parameter recovery, incurs all these 338 errors.
Radare2/Ghidra can also miss to identify certain local variables. Root cause
analysis shows that due to bugs in type recovery module of Radare2 (i.e.,
Bug$_{8}$), variable is incorrectly assigned with a larger size (e.g., a 32-bit
integer). Variables adjacent to this ``larger'' variable can overlap in the
memory layout, and can be potentially deemed as part of this ``larger'' variable
and is therefore optimized out.

We also find seven erroneous variable recoveries in JEB3 which causes
``undefined behavior'' in the decompiled C code. Consider a simplified case:

\begin{lstlisting}
  unsigned int v0;
  unsigned int v1 = v0 >> 16;
\end{lstlisting}

\noindent where \texttt{v0} is defined yet uninitialized, leading to an
indeterminate value in \texttt{v1}. We have confirmed that the source code does
not contain any uninitialized local variables. In general, generating code with
undefined behavior is undesired for decompilers. Although the root cause is yet
to be determined, we suspect that \texttt{v0} in the above case is hardcoded in
the output. We urge the decompiler developers to avoid generating code
exhibiting undefined behavior, for instance, by initializing \texttt{v0} with
zero.

\subsubsection{Control-Flow Recovery}
\label{subsubsec:structure-recovery}
We find a total of 52 deviant outputs due to control-flow errors in the
decompiled C code. We note that after taking a close look at the buggy code
fragments, \textit{all} failures in RetDec and Radare2/Ghidra are actually due
to wrong type recovery and optimization bugs. Consider a simplified input
program below:

\begin{lstlisting}
 // condition generated by EMI 
 if (opaque_condition){ // evaluated to false 
   statement1; // not reachable
 }
\end{lstlisting}
\noindent where the \texttt{opaque\_condition} will be evaluated to false during
runtime. However, we report that the \texttt{if} condition was optimized out in
the decompiled program since the condition is incorrectly evaluated to ``true''
due to type recovery or optimization errors. Hence, the unreachable branch
becomes reachable, reflecting a ``control-structure'' error in the decompiled C
code. We report that Bug$_{3-4}$ found in RetDec and Bug$_{9-13}$ in
Radare2/Ghidra all lead to such issues, although they represent different buggy
code fragments in the type recovery and optimization modules.

We also find issues where the statements are mistakenly reordered in IDA-Pro
outputs. Consider the case below:

\vspace{3pt}
\noindent\begin{minipage}{.50\linewidth}
\begin{lstlisting}
// source code
 if (cond1)
   statement1; 
 if (cond2)
   statement2; 
\end{lstlisting}
\end{minipage}\hspace*{12pt}
\begin{minipage}{.50\linewidth}
\begin{lstlisting}
// decompiled code
 if (cond2)
   statement2; 
 if (cond1)
   statement1; 
\end{lstlisting}
\end{minipage}

\noindent where in the decompiled outputs, two \texttt{if} statements are
reordered, altering execution flow, and leading to deviant execution outputs.

\subsubsection{Optimization}
\label{subsubsec:optimization}
Academic researchers design decompiler optimizations to make decompiled code
close to the input source code and thus more
``readable''~\cite{brumley2013native,yakdan2015no}. However, optimizations,
particularly the erroneous constant folding and constant propagation, can make
decompiled C code mal-functional. As aforementioned, from the 13 bugs reported
in \T~\ref{tab:root}, six are within the optimization modules of decompilers,
for instance performing constant folding without correctly taking bit length
into account (Bug$_{5}$), or incorrectly using a 32-bit ghost variable defined
in Ghidra to replace a 16-bit variable during constant propagation (Bug$_{11}$).

In addition to errors, we note that the overly (and wrongly) optimized C code
often becomes \textit{too concise}. Such aggressive optimization has diminished
the readability of decompiled C code to a great extent, and has caused a major
challenge for our manual inspection (\S~\ref{subsec:root}). While
``readability'' could be a subjective criterion, inspired by our observation, we
measure the readability by 1) reporting the average LOC for the decompiled code,
and 2) analyzing the code similarity between the decompiled outputs and the
input programs. We leverage a popular software similarity analyzer,
\texttt{moss}~\cite{moss}, to measure code similarity. The similarity score
(ranging from 0 to 1.0; higher is better) indicates how close the decompiled
outputs and inputs are. The results are reported as follows:

\begin{table}[H]
	\centering
	\scriptsize
  \resizebox{0.95\linewidth}{!}{
  \begin{tabular}{c|c|c|c|c}
	\hline
  & \textbf{IDA-Pro} & \textbf{JEB3} & \textbf{RetDec} & \textbf{Radare2/Ghidra} \\
	\hline
	LOC              & 90   & 85   & 54   & 104 \\
	Similarity Score & 0.51 & 0.50 & 0.54 & 0.49 \\
	\hline
\end{tabular}
}
\end{table}

Decompiled programs are highly concise, in the sense that their average LOC is
much lower than the corresponding LOC of input programs (on average 143; see
\T~\ref{tab:data}). Even worse, the average similarity score between decompiled
outputs and input programs is also low. In summary, we interpret that the
highly-optimized decompiled outputs obstruct the readability notably (see
further discussions in \S~\ref{subsec:emi-implication}).

Also, the above results may (incorrectly) indicate that decompilers
``consistently'' optimize their outputs, since their average similarity scores
w.r.t. reference inputs are close. Nevertheless, \S~\ref{sec:discussion} will
show that indeed for an input executable, its corresponding outputs of four
decompilers have very different representations, indicating a strong need for
regulating optimization and code generation.

\subsection{Others}
\label{subsec:others}
We find six errors in the ``Others'' category: we report that the decompiled
outputs have syntax-level difference (e.g., arithmetic operators) compared with
the input source code. While the root cause is unknown (since these two
decompilers are closed source), we suspect such issues are due to sloppy errors
in the C statement translation stage, which could be fixed by developers easily.

\subsection{Result Implication}
\label{subsec:emi-implication}
In this section, we present discussion and result implication to answer research
question \textbf{RQ3}: \textit{what insights can we deduce from analyzing the
  decompilation defects?}
\\\\
\noindent \textbf{Support of Cutting-Edge Research Outputs.} We have found
plenty of type, variable, and control structure errors in the decompiled C code,
and explained their corresponding buggy fragments in the decompilers. Although
academic researchers are believed to have mostly addressed such reverse
engineering challenges (since we are evaluating non-trivial but \textit{not
  extreme} cases), one observation is that modern decompilers have not fully
implemented those well-established research products. For instance, while the
state-of-the-art research has been working on function prototype recovery for
years and achieved promising results (e.g., close to 99\% accuracy for function
recognition in x86
binaries~\cite{bao2014byteweight,shin2015recognizing,zheng2017neutral}), still,
the de facto decompilers (e.g., RetDec) have not implemented the proposed
methods and therefore make lots of errors in recovering function prototypes and
parameters. Also, recovering types from x86 binary code have been formulated as
a recursively-constrained type inference approach with sub-typing, recursive
types, and polymorphism~\cite{lee2011tie,noonan2016poly}. Contrarily, C
decompilers, from the disclosed documents and our observation, only implement
simple inference techniques combined with heuristics and predefined
patterns~\cite{kvroustek2017retdec,guilfanov2001type,jebtype}.

\begin{quote}
\textbf{Finding:} The de facto decompilers still have not fully leveraged the
research outputs in this field to improve reverse engineering accuracy.
\end{quote}

Although research products cannot be used to address every corner case, most
defects exposed in this study, such as RetDec's obvious limit in recovering
function prototypes, shall be fixed smoothly. Overall, while modern decompilers
perform decently in recovering high-level source code, we urge developers to
embrace research products in this field to revamp the design and solve problems
exposed in this study.
\\\\
\noindent \textbf{Optimization.}~As disclosed in
\S~\ref{subsubsec:optimization}, our study on de facto decompilers uncovers the
following finding:

\begin{quote}
\textbf{Finding:} De facto decompilers extensively simplify their outputs, even
though readability and decompilation correctness are undermined simultaneously.
\end{quote}

We encountered major difficulty when manually inspecting erroneous outputs that
are highly simplified. We suspect that if it was not even presentable for us ---
reverse engineering analysts --- to comprehend the decompiled outputs, it should
be accurate to assume the outputs are often not readable enough for layman
users. This clearly indicates a \textit{mismatch} between expectations in the
literature and the actual capabilities of modern decompilers. Note that in
academia, the optimization module of decompilers is designed following the
principle of \textit{enhancing} the readability and making it close to the
original C code~\cite{brumley2013native,yakdan2015no}.

Although optimization can help to simplify code emitted by decompilation passes
and can usually output one succinct high-level statement by folding several
statements, we advocate fine-grained calibration. Currently, modern decompilers
seem to go too far and notably hurt readability of their outputs. Meanwhile,
motivated by how compiler optimizations are provided for usage, we urge
decompiler developers to make their products configurable to flexibly select
optimization passes.


==> llvmir.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=1.00\linewidth]{fig/llvmir.pdf}
  \caption{Comparison between LLVM IR generated from sample C code with IR
    lifted from binary code compiled from the C code. The sample C code is
    presented on the lower right corner. LLVM IR code is simplified due to the
    limited space and the \texttt{main} function is backgrounded with
    \colorbox{gray!30}{grey} for better readability.}
  \label{fig:llvmir}
\end{figure*}



==> motivation.tex <==
\section{Motivation}
\label{sec:motivation}

In this section, we show the research topic is \textit{central} and
\textit{timely}, by shedding light on potential mismatches between traditional
conservative stance of using decompiled C code and the progressive development
of decompilation techniques. We also discuss the pitfalls of leveraging IRs for
binary code analysis to advocate the development of decompilation techniques.

\begin{figure*}[t]
\centering
%\vspace{1pt}
\includegraphics[width=1.00\linewidth]{fig/motivating-example.pdf}
%\vspace{-15pt}
\caption{Motivating example of generating code completion outputs for a LeetCode
snippet and two mutated versions using Copilot.}
\label{fig:motivating}
\end{figure*}
